On Cohen-Jones isomorphism in string topology

The loop product is an operation in string topology. Cohen and Jones gave a homotopy theoretic realization of the loop product as a classical ring spectrum $LM^{-TM}$ for a manifold $M$. Using this, they presented a proof of the statement that the loop product is isomorphic to the Gerstenhaber cup product on the Hochschild cohomology $HH^*(C^*(M)\,;C^*(M))$ for simply connected $M$. However, some parts of their proof are technically difficult to justify. The main aim of the present paper is to give detailed modification to a geometric part of their proof. To do so, we set up an "up to higher homotopy" version of McClure-Smith's cosimplicial product. We prove a structured version of Cohen-Jones isomorphism in the category of symmetric spectra.

==> psi2.tex <==
%WinTpicVersion4.32a
{\unitlength 0.1in%
\begin{picture}(35.2000,97.3000)(0.9000,-98.1000)%
% CIRCLE 2 0 3 0 Black White  
% 4 1114 2405 1874 1081 2000 1151 250 1161
% 
\special{pn 8}%
\special{ar 1114 2405 1527 1527 4.1053411 5.3274901}%
% CIRCLE 2 0 3 0 Black White  
% 4 3610 9810 3610 9810 2050 5550 5190 5900
% 
\special{pn 8}%
\special{ar 3610 9810 0 0 5.0964180 4.3613581}%
% CIRCLE 2 0 3 0 Black White  
% 4 3600 9160 3600 9160 3600 9160 6180 6410
% 
\special{pn 8}%
\special{ar 3600 9160 0 0 5.4659030 6.2831853}%
% CIRCLE 2 0 3 0 Black White  
% 4 1110 2395 2290 465 2064 355 80 355
% 
\special{pn 8}%
\special{ar 1110 2395 2262 2262 4.2448275 5.1498209}%
% VECTOR 0 0 3 0 Black White  
% 2 810 995 1404 305
% 
\special{pn 20}%
\special{pa 810 995}%
\special{pa 1404 305}%
\special{fp}%
\special{sh 1}%
\special{pa 1404 305}%
\special{pa 1345 342}%
\special{pa 1369 345}%
\special{pa 1376 369}%
\special{pa 1404 305}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 814 995 840 1015 840 1015 840 1015
% 
\special{sh 1.000}%
\special{ia 814 995 33 33 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 814 995 33 33 0.0000000 6.2831853}%
% CIRCLE 2 0 0 0 Black Black  
% 4 1430 281 1424 315 1424 315 1424 315
% 
\special{sh 1.000}%
\special{ia 1430 281 35 35 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 1430 281 35 35 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black Black  
% 2 1430 281 1430 1101
% 
\special{pn 8}%
\special{pa 1430 281}%
\special{pa 1430 1101}%
\special{fp}%
% LINE 2 0 3 0 Black Black  
% 2 1430 1091 1584 1091
% 
\special{pn 8}%
\special{pa 1430 1091}%
\special{pa 1584 1091}%
\special{fp}%
% BOX 2 0 3 0 Black Black  
% 2 1430 1091 1490 1031
% 
\special{pn 8}%
\special{pa 1430 1091}%
\special{pa 1490 1091}%
\special{pa 1490 1031}%
\special{pa 1430 1031}%
\special{pa 1430 1091}%
\special{pa 1490 1091}%
\special{fp}%
% CIRCLE 2 0 0 0 Black Black  
% 4 1414 1111 1430 1085 1430 1085 1430 1085
% 
\special{sh 1.000}%
\special{ia 1414 1111 31 31 0.0000000 6.2831853}%
\special{pn 8}%
\special{ar 1414 1111 31 31 0.0000000 6.2831853}%
% LINE 2 0 3 0 Black White  
% 2 1134 615 884 615
% 
\special{pn 8}%
\special{pa 1134 615}%
\special{pa 884 615}%
\special{fp}%
% STR 2 0 3 0 Black White  
% 4 470 565 470 615 5 0 0 0
% $v-\phi(v_i)$
\put(4.7000,-6.1500){\makebox(0,0){$v-\phi(v_i)$}}%
% STR 2 0 3 0 Black White  
% 4 680 1105 680 1155 5 0 0 0
% $\phi(y)$
\put(6.8000,-11.5500){\makebox(0,0){$\phi(y)$}}%
% STR 2 0 3 0 Black White  
% 4 1674 391 1674 441 5 0 0 0
% $\widehat{\psi}(d)(y)$
\put(16.7400,-4.4100){\makebox(0,0){$\widehat{\psi}(d)(y)$}}%
% STR 2 0 3 0 Black White  
% 4 1424 1191 1424 1241 5 0 0 0
% $\psi(d)(y)$
\put(14.2400,-12.4100){\makebox(0,0){$\psi(d)(y)$}}%
% STR 2 0 3 0 Black White  
% 4 2090 95 2090 145 5 0 0 0
% $\nu_\eps(\phi)$
\put(20.9000,-1.4500){\makebox(0,0){$\nu_\eps(\phi)$}}%
% STR 2 0 3 0 Black White  
% 4 1980 975 1980 1025 5 0 0 0
% $\phi(M)$
\put(19.8000,-10.2500){\makebox(0,0){$\phi(M)$}}%
\end{picture}}%

